Single W and Z boson production properties and asymmetries

Recent analyses of single $W$ and $Z$ boson production properties and asymmetries from the CDF and D\O\ experiments at the Fermilab Tevatron are reported. For $W$ boson production, measurements of the production and lepton charge asymmetries are presented. For $Z/\gamma^*$ production, the following measurements are presented: $d\sigma/dy$, $(1/\sigma) (d\sigma/dp_T)$, $(1/\sigma) (d\sigma/d\phistar)$, lepton angular coefficients, and $A_{FB}$ with extraction of $\sin^2\theta_W$ and the light quark couplings to the $Z$. Most of these measurements are in good agreement with QCD predictions.

==> plots/AFB_CDF/extract-eps <==
eval '(exit $?0)' && eval 'exec perl -S $0 ${1+"$@"}' && eval 'exec perl -S $0 $argv:q' if 0;

# Usage: extract-eps [-a] [-l] [-n] [-fig] [ps-files ...]
#                                                         --gnome

# ... 1: always overwrite, 0: ask, -1: never overwrite
$overwrite = 0;
$listonly = 0;
$add_figno = 0;
$have_ps2epsi = 1;
$tmpfile = ".tmpextract.eps";
$needhelp = 0;
foreach $text (@ARGV)  {
  last if (!($text=~/^-/));
  if ($text=~/-a/) {$overwrite = 1}
  elsif ($text=~/-n/) {$overwrite = -1}
  elsif ($text=~/-l/) {$listonly = 1}
  elsif ($text=~/-fig/) {$add_figno = 1}
  elsif ($text=~/-[\?hH]/) {goto HELP}
  else {print "Unrecognized option $text \n"; $need_help = 1};
  shift(@ARGV);
}
goto HELP if ($need_help);

$epsfile_open = 0;
$figno = 0;
$oldfile = '000000';
while (<>) {
  if ($oldfile ne $ARGV) {
    $oldfile = $ARGV;
    $text = $listonly ? "Listing" : "Extracting" ;
    print "\n$text eps files ", (($ARGV ne "-") ? "from $oldfile " : ""), "...\n";}
  if (!$epsfile_open) {
    next if (!/^%%BeginDocument:/);
    ($epsfile) = /^%%BeginDocument:\s*(\S+)/;
    if ($epsfile=~/\//) {$epsfile =~ s/.*\///;}
    ++$figno;
    if ($add_figno) {$epsfile = "fig$figno-$epsfile"};
    if ($listonly) {
      print "    Found file $epsfile \n";
      next;
    }
    if (-e $epsfile) {
      next if ($overwrite < 0);
      if ($overwrite == 0) {
        print " >>> File $epsfile already exists, overwrite? [<CR>=no] ";
        $text = <STDIN>;
        $overwrite = 1 if ($text=~/^\s*Y/);
        $overwrite = -1 if ($text=~/^\s*N/);
        next if (!($text=~/^\s*y/i));
      }
    }
    open (EPS,">$epsfile");
    $epsfile_open = 1;
  } else {
    if (!/^%%EndDocument/) {print EPS "$_" ; next}
    close (EPS);
    print "    Extracted file $epsfile";
    $epsfile_open = 0;
    if (!$have_ps2epsi) {print "\n"; next}; 
    eval `ps2epsi $epsfile $tmpfile`;
    if ($@) {$have_ps2epsi = 0} 
    else {eval `mv $tmpfile $epsfile`; print " ... created bounding box"};
    print "\n";
  }
}
print "Done.\n\n";
if (!$have_ps2epsi) {
  print "NOTE: could not create bounding boxes with ps2epsi.\n\n"}
exit(0);

HELP:
print "\nUsage:   extract-eps [-a] [-n] [-l] [ps_files ...]\n";
print "\n  -a       : always overwrite existing eps files";
print "\n  -n       : never overwrite existing eps files";
print "\n  -l       : only list eps files, do not extract";
print "\n  -fig     : prefix extracted eps filenames with fig#";
print "\n  ps_files : postscript taken from STDIN if ps_files not provided \n";
print "\n"; exit(0);

